A Systematic Survey of the Effects of Wind Mass Loss Algorithms on the Evolution of Single Massive Stars

Mass loss is a key uncertainty in the evolution of massive stars. Stellar evolution calculations must employ parametric algorithms for mass loss, and usually only include stellar winds. We carry out a parameter study of the effects of wind mass loss on massive star evolution using the open-source stellar evolution code MESA. We provide a systematic comparison of wind mass loss algorithms for solar-metallicity, nonrotating, single stars in the initial mass range of $15-35\,M_\odot$. We consider combinations drawn from two hot phase algorithms, three cool phase algorithms, and two Wolf-Rayet algorithms. We consider linear wind efficiency scale factors of $1$, $0.33$, and $0.1$ to account for reductions in mass loss rates due to wind inhomogeneities. We find that the initial to final mass mapping for each zero-age main-sequence (ZAMS) mass has a $\sim 50\%$ uncertainty if all algorithm combinations and wind efficiencies are considered. The ad-hoc efficiency scale factor dominates this uncertainty. While the final total mass and internal structure of our models vary tremendously with mass loss treatment, final observable parameters are much less sensitive for ZAMS mass $\lesssim 30\,M_\odot$. This indicates that uncertainty in wind mass loss does not negatively affect estimates of the ZAMS mass of most single-star supernova progenitors from pre-explosion observations. Furthermore, we show that the internal structure of presupernova stars is sensitive to variations in both main sequence and post main-sequence mass loss. We find that the compactness parameter $\xi\propto M/R(M)$ varies by as much as $30\%$ for a given ZAMS mass evolved with different wind efficiencies and mass loss algorithm combinations. [abridged]

==> table_O_depl.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "AA_mmps"
%%% End: 


\begin{table*}[!ht]
    \centering
    % \caption{Radius ($R$), total mass
    %   ($M_\mathrm{tot}$), He core mass
    %   ($M_\mathrm{He}$) and CO core
    %   mass ($M_\mathrm{CO}$) in solar units, and compactness parameter
    %   $\xi_{2.5}$ for the models run until oxygen depletion, i.e.\ $X_c(\mathrm{^{16}O})<0.04$ and
    %   $X_c(\mathrm{^{28}Si})>0.01$. These runs are re-started from the
    %   corresponding MESA model saved at the "end of the mass loss
    %   phase", when $T_c\geq10^9\,\mathrm{K}$. Note that the value of
    %   $M_\mathrm{CO}$ for the model s30VdJNL$\_$1.0 has been obtained
    %   visually from the abundances profile $X_i\equiv X_i(M)$,
    %   because the threshold to define the CO core boundary in MESA is
    %   never reached within this model. See \todo{cite thesis} for a
    %   definition of the core boundaries easier to generalize in these
    %   situations, which has not been adopted here to facilitate the comparison with
    %   previous calculations.
    % }
    \caption{Stellar properties at Oxygen depletion, 
      i.e.\ $X_c(\mathrm{^{16}O})<0.04$ and
      $X_c(\mathrm{^{28}Si})>0.01$. 
      The last column shows the maximum difference in $\xi_{2.5}$ for each value of $\eta$.
      These runs are re-started from the
      corresponding MESA models saved at the "end of the mass loss
      phase", when $T_c\geq10^9\,\mathrm{K}$. % SAID BEFORE: Note that the value of
      % $M_\mathrm{CO}$ for the $M_\mathrm{ZAMS}=30\,M_\odot$ computed with $\eta=1.0$ and VdJNL
      % is obtained visually from the abundances profile $X_i\equiv X_i(M)$. This is 
      % because the threshold to define the CO core boundary in MESA is
      % never reached within this model. See \todo{cite thesis} for a
      % definition of the core boundaries easier to generalize in these
      % situations, which has not been adopted here to facilitate the comparison with
      % previous calculations.
      % \todo{fix last sentence: send plot to Christian}
      \label{tab:runs_to_O_depl}} 
    \begin{tabular}{c|cl|cccccc}\hline \hline
      \multicolumn{8}{c}{Oxygen depletion: $X_c(\mathrm{^{16}O})<0.04$ and $X_c(\mathrm{^{28}Si})>0.01$}\\\hline\hline
      $M_\mathrm{ZAMS} \ [M_\odot]$ & $\eta$ &  \multicolumn{1}{c|}{\phantom{A}wind ID}  & $R \ [R_\odot]$ &
      $M_\mathrm{tot} \ [M_\odot]$ & $M_\mathrm{He} \ [M_\odot]$ &
      $M_\mathrm{CO} \ [M_\odot]$ & $\xi_{2.5}$ & $\max \Delta
        \xi_{2.5} $\\\hline\hline
      \multirow{9}{*}{15} & \multirow{3}{*}{0.1\phantom{3}} & \phantom{A}VdJNL & \phantom{0}908 & 14.66 & \phantom{0}4.99 & 3.17 & 0.155  & \multirow{3}{*}{0.001}\\ 
                          &                                 & \phantom{A}VvLNL & \phantom{0}924 & 13.60 & \phantom{0}4.98 & 3.17 & 0.156  &                        \\ 
                          &                                 & \phantom{A}KNJNL & \phantom{0}911 & 14.66 & \phantom{0}5.00 & 3.17 & 0.156  &                        \\ 
      \cline{2-9}                               
                          & \multirow{2}{*}{0.33}           & \phantom{A}VNJNL & \phantom{0}914 & 13.90 & \phantom{0}4.93 & 3.13 & 0.153  & \multirow{2}{*}{0.001}\\ 
                          &                                 & \phantom{A}VvLNL & \phantom{0}967 & 10.39 & \phantom{0}4.93 & 3.13 & 0.152  &                       \\ 
      \cline{2-9}                                                              
                          & \multirow{4}{*}{1.0\phantom{3}} & \phantom{A}VNJNL & \phantom{0}895 & 12.74 & \phantom{0}4.65 & 2.95 & 0.141  & \multirow{4}{*}{0.014} \\ 
                          &                                 & \phantom{A}VvLNL & \phantom{0}629 & \phantom{0}5.25 & \phantom{0}4.64 & 2.94 & 0.139 &\\ 
                          &                                 & \phantom{A}KNJNL & \phantom{0}946 & 11.87 & \phantom{0}4.92 & 3.12 & 0.153 & \\ 
                          &                                 & \phantom{A}KvLNL & \phantom{0}643 & \phantom{0}5.70 & \phantom{0}4.90 & 3.11 & 0.152 &\\ 
      \hline\hline       
      \multirow{12}{*}{20}& \multirow{4}{*}{0.1\phantom{3}} & \phantom{A}VdJNL & \phantom{0}994 & 19.23 & \phantom{0}7.04 & 4.83 & 0.182& \multirow{4}{*}{0.007}\\ 
                          &                                 & \phantom{A}VvLNL & \phantom{0}998 & 18.10 & \phantom{0}7.03 & 4.83 & 0.178&\\ 
                          &                                 & \phantom{A}KNJNL & \phantom{0}991 & 19.37 & \phantom{0}7.01 & 4.82 & 0.179&\\ 
                          &                                 & \phantom{A}KvLNL & \phantom{0}991 & 18.67 & \phantom{0}7.01 & 4.82 & 0.175&\\ 
                          \cline{2-9}                               
                          & \multirow{4}{*}{0.33}           & \phantom{A}VNJNL &   1001 & 17.48 & \phantom{0}7.01 & 4.81 & 0.161& \multirow{4}{*}{0.052}\\ 
                          &                                 & \phantom{A}VvLNL & \phantom{0}987 & 13.47 & \phantom{0}6.99 & 4.80 & 0.175&\\ 
                          &                                 & \phantom{A}KdJNL & \phantom{0}999 & 17.62 & \phantom{0}7.00 & 4.80 & 0.213&\\ 
                          &                                 & \phantom{A}KvLNL & \phantom{0}993 & 13.90 & \phantom{0}6.98 & 4.80 & 0.175&\\ 
                          \cline{2-9}                                  
                          & \multirow{4}{*}{1.0\phantom{3}}  & \phantom{A}VdJNL & \phantom{0}951 & 11.81 & \phantom{0}7.06 & 4.85 & 0.182& \multirow{4}{*}{0.010}\\ 
                          &                                 & \phantom{A}VvLNL & \phantom{0}673 & \phantom{0}8.80 & \phantom{0}7.02 & 4.82 & 0.176&\\ 
                          &                                 & \phantom{A}KNJNL & \phantom{0}978 & 12.77 & \phantom{0}6.95 & 4.77 & 0.176&\\ 
                          &                                 & \phantom{A}KvLNL & \phantom{0}712 & \phantom{0}8.81 & \phantom{0}6.90 & 4.73 & 0.172&\\ 
      \hline\hline                                 
      \multirow{11}{*}{25}& \multirow{4}{*}{0.1\phantom{3}} & \phantom{A}VdJNL & \phantom{0}898 & 23.85 & \phantom{0}9.14 & 6.46 & 0.180& \multirow{4}{*}{0.023}\\ 
                          &                                 & \phantom{A}VvLNL & \phantom{0}899 & 23.56 & \phantom{0}9.14 & 6.44 & 0.179&\\ 
                          &                                 & \phantom{A}KNJNL & \phantom{0}888 & 23.76 & \phantom{0}9.24 & 6.52 & 0.159&\\ 
                          &                                 & \phantom{A}KvLNL & \phantom{0}889 & 23.24 & \phantom{0}9.23 & 6.50 & 0.157&\\ 
                          \cline{2-9}                                                 
                          & \multirow{3}{*}{0.33}           & \phantom{A}VNJNL & \phantom{0}922 & 22.02 & \phantom{0}8.87 & 6.25 & 0.161& \multirow{3}{*}{0.049} \\ 
                          &                                 & \phantom{A}VvLNL & \phantom{0}929 & 22.13 & \phantom{0}8.87 & 6.20 & 0.164&\\ 
                          &                                 & \phantom{A}KdJNL & \phantom{0}894 & 21.27 & \phantom{0}9.11 & 6.42 & 0.210&\\ 
                          \cline{2-9}                               
                          & \multirow{4}{*}{1.0\phantom{3}} & \phantom{A}VNJNL & \phantom{0}812 & 13.67 & \phantom{0}9.05 & 6.32 & 0.164& \multirow{4}{*}{0.050} \\ 
                          &                                 & \phantom{A}VvLNL & \phantom{0}786 & 12.97 & \phantom{0}9.04 & 6.29 & 0.211&\\ 
                          &                                 & \phantom{A}KdJNL & \phantom{0}875 & 15.57 & \phantom{0}8.89 & 6.21 & 0.161&\\ 
                          &                                 & \phantom{A}KvLNL & \phantom{0}860 & 14.69 & \phantom{0}8.90 & 6.23 & 0.200&\\ 
                          \hline\hline       
      \multirow{11}{*}{30}& \multirow{4}{*}{0.1\phantom{3}} & \phantom{A}VdJNL& \phantom{0}701 & 28.11 & 10.97 & 7.89 & 0.242& \multirow{4}{*}{0.001}\\ 
                          &                                 & \phantom{A}VNJNL& \phantom{0}697 & 28.17 & 10.97 & 7.90 & 0.243&\\ 
                          &                                 & \phantom{A}KNJNL& \phantom{0}706 & 28.19 & 10.91 & 7.83 & 0.242&\\ 
                          &                                 & \phantom{A}KvLNL& \phantom{0}719 & 28.75 & 10.90 & 7.74 & 0.242&\\ 
                          \cline{2-9}                                            
                          & \multirow{4}{*}{0.33}           & \phantom{A}VdJNL& \phantom{0}668 & 24.16 & 11.11 & 7.99 & 0.243& \multirow{4}{*}{0.023} \\ 
                          &                                 & \phantom{A}VvLNL& \phantom{0}723 & 26.02 & 11.10 & 8.00 & 0.243& \\ 
                          &                                 & \phantom{A}KNJNL& \phantom{0}716 & 25.18 & 10.89 & 7.85 & 0.228& \\ 
                          &                                 & \phantom{A}KvLNL& \phantom{0}709 & 27.12 & 10.87 & 7.79 & 0.220& \\ 
                          \cline{2-9}                               
                          & \multirow{3}{*}{1.0\phantom{3}}  & \phantom{A}VdJNL& \phantom{0}610 & 15.36 & 11.28 & 8.20 %2.16
                                                                                                & 0.179 & \multirow{3}{*}{0.065}           \\ 
                          &                                 & \phantom{A}KdJNL& \phantom{0}756 & 18.51 & 10.92 & 7.85 & 0.244&\\ 
                          &                                 & \phantom{A}KvLNL& \phantom{0}723 & 22.53 & 10.89 & 7.74 & 0.243&\\ 
    \end{tabular}
  \end{table*}


==> table_onset_cc.tex <==
\begin{table*}[!htb]
\centering
\caption{Properties of the subset of models run up to the onset of
  core collapse, $\mathrm{max}\{ |v| \} \geq 10^3 \ \mathrm{km \
    s^{-1}}$ (see \Eqref{eq:onset_cc}). $M_4 \udef M(s=4)$ is the mass
  enclosed within the location where the specific entropy $s<4 \
  \mathrm{N_A k_b}$, $\mu_4\udef dm/dr|_{s=4}$ is the mass gradient at
  this location \citep[see][]{ertl:15}, $M_{\rho_6} \udef M(\rho = 10^6
  \mathrm{g \ cm^{-3})}$ is the mass enclosed in the location where
  the density drops below $10^6 \ \mathrm{g \ cm^{-3}}$,
  $M_\mathrm{CO}$ and $M_\mathrm{Fe}$ are the
   carbon-oxygen and iron core masses, respectively. 
   % SAID BEFORE: Note that we do
   % not require a minimum abundance of either carbon or oxygen in the
   % CO core (in contrast with the MESA defaults, which yield a null
   % carbon core).
   \label{tab:onset_cc}}
\begin{tabular}{c|cl|cccccc}
  \hline
  \hline
  \multicolumn{9}{c}{Onset of core collapse: $\mathrm{max}\{ |v| \} \geq 10^3 \ \mathrm{km \ s^{-1}}$ }\\
  \hline
  \hline
  $M_\mathrm{ZAMS} \ [M_\odot]$ & $\eta$ & \multicolumn{1}{l|}{wind ID}  & $ \xi_{2.5}^\mathrm{pre-SN}$ & $M_4 \ [M_\odot] $ & $\mu_4$ & $M_{\rho_6} \ [M_\odot]$ &  $M_\mathrm{CO} \ [M_\odot]$ & $M_\mathrm{Fe} \ [M_\odot]$ \\\hline\hline 
  \multirow{2}{*}{15} & \multirow{2}{*}{1.0} & VNJNL & 0.103 & 1.71 & 0.045 & 1.68 &  2.91 & 1.39\\ 
                      &                      & KvLNL & 0.132 & 1.78 & 0.051 & 1.79 &  3.07 & 1.50\\ 
  \hline
  \multirow{2}{*}{25} & \multirow{2}{*}{0.33} & VvLNL & 0.227 & 1.73 & 0.084 & 1.84 &  6.38 & 1.51\\ 
                      &                       & KdJNL & 0.308 & 2.05 & 0.100 & 2.19 &  6.40 & 1.63\\ 
  \hline
  \multirow{2}{*}{30} & \multirow{2}{*}{0.33} & VdJNL & 0.358 & 1.60 & 0.163 & 2.21  & 7.98 & 1.56\\ 
                      &                       & KNJNL & 0.276 & 1.82 & 0.100 & 1.98 &  7.90 & 1.58\\ 

\hline
\end{tabular}
\end{table*}


==> table_scaling.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "AA_mmps"
%%% End: 


\begin{table*}[!ht]
\setlength{\abovecaptionskip}{-0.1cm}
\setlength{\belowcaptionskip}{-0.2cm}
\begin{center}
\caption{$\dot{M}$ scaling with physical quantities (luminosity $L$,
  mass $M$, escape velocity $v_\mathrm{esc}$ and final velocity
  $v_\infty$ of the wind, thermal velocity $v_\mathrm{th}$, effective
  temperature $T_\mathrm{eff}$, 
  radius $R$, Eddington ratio $\Gamma_\mathrm{E} =
  L/L_\mathrm{Edd}$, surface hydrogen and helium abundances and
  metallicity, 
  $X_s$,
$Y_s$, and $Z_s$, respectively). 
The scaling are obtained from the algorithms
described in \Secref{app:schemes_review}, and errors and overall
multiplying factors are
omitted for the sake of brevity. See \Tabref{tab:comb} for the naming
convention for mass loss algorithm combinations. \label{tab:scaling} }

\newcommand{\mc}[3]{\multicolumn{#1}{#2}{#3}}
\renewcommand{\arraystretch}{2.5}
\begin{tabular}{c|c|c|c|c|c|c}
\hline\hline
ID & VdJNL & VNJNL & VvLNL & VdJH & VNJH & VvLH \\\hline
\multirow{2}{*}{Hot} &
\mc{6}{l}{$L^{2.210}M^{-1.339}\left(\frac{v_\infty}{2v_\mathrm{esc}}\right)^{-1.601}T_\mathrm{eff}^{1.07}Z^{0.85}$\phantom{aaaaaaaaaaaaaaaa}
  \hfill if $T_\mathrm{eff} < 22.5 \ \mathrm{kK}$}  \\
 & \mc{6}{l}{$L^{2.194}M^{-1.313}\left(\frac{v_\infty}{2v_\mathrm{esc}}\right)^{-1.226}Z^{0.85}T_\mathrm{eff}^{(0.933-10.92\log(T_\mathrm{eff}/
     40 \mathrm{kK}))}$ \hfill if $T_\mathrm{eff} > 27.5 \ \mathrm{kK}$} \\\hline
Cool & $L^{1.769}T_\mathrm{eff}^{-1.676}$ & $L^{1.24}M^{0.16}R^{0.81}$
& $L^{1.05}T_\mathrm{eff}^{-6.3}$& $L^{1.769}T_\mathrm{eff}^{-1.676}$ & $L^{1.24}M^{0.16}R^{0.81}$
& $L^{1.05}T_\mathrm{eff}^{-6.3}$ \\\hline
 \multirow{2}{*}{WR}& \mc{3}{l}{\multirow{2}{*}{$L^{1.29}Y_s^{1.73}Z_s^{0.47}$}}\hfill &
 \mc{3}{|l}{$L^{1.5}10^{-2.85X_s}$ \hfill if $\log_{10}(L/L_\odot)>4.5$} \\
 & \mc{3}{l}{} & \mc{3}{|l}{$L^{6.8}$\phantom{aaaaaaaa} \hfill if $\log_{10}(L/L_\odot)\leq4.5
   $}\\\hline\hline
ID & KdJNL & KNJNL & KvLNL & KdJH & KNJH & KvLH \\\hline
Hot  &
\mc{6}{l}{$L^{1.779}v_\mathrm{th}^{-1.169}[GM(1-\Gamma_\mathrm{E})]^{0.610}$}\hfill\\\hline
Cool & $L^{1.769}T_\mathrm{eff}^{-1.676}$ & $L^{1.24}M^{0.16}R^{0.81}$
& $L^{1.05}T_\mathrm{eff}^{-6.3}$& $L^{1.769}T_\mathrm{eff}^{-1.676}$ & $L^{1.24}M^{0.16}R^{0.81}$
& $L^{1.05}T_\mathrm{eff}^{-6.3}$ \\\hline
 \multirow{2}{*}{WR}&  \mc{3}{l}{\multirow{2}{*}{$L^{1.29}Y_s^{1.73}Z_s^{0.47}$}}\hfill &
 \mc{3}{|l}{$L^{1.5}10^{-2.85X_s}$ \hfill if $\log_{10}(L/L_\odot)>4.5$}\\
 & \mc{3}{l}{} & \mc{3}{|l}{$L^{6.8}$\phantom{aaaaaaaa} \hfill if $\log_{10}(L/L_\odot)\leq4.5$}\\
\end{tabular}
\end{center}
\end{table*}


==> table_simple_scaling.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

\begin{table}[!b]
\setlength{\abovecaptionskip}{-0.1cm}
\setlength{\belowcaptionskip}{-0.2cm}
\begin{center}
\caption{Scaling of the \newtext{mass loss rate} $\dot{M}$ predicted by different algorithms
  with luminosity and effective temperature. We refer the reader to
  \Tabref{tab:scaling}, \Secref{app:schemes_review} and references
  therein for the detailed formulae implemented in MESA and the
  complete scaling. \label{tab:scalingLT}}
\begin{tabular}{l|cc}\hline\hline
  \multicolumn{3}{c}{\large  $\log(\dot{M})\propto \alpha\log(L)+\beta\log(T_\mathrm{eff})$} \\\hline\hline
  \multicolumn{1}{l|}{ID} & $\alpha$  & $\beta$       \\ \hline\hline
  V                       & $\sim$2.2 & $\sim$1.0     \\
  K                       & $\sim$1.2 & $\sim$0.6     \\
  \hline
  dJ                      & $\sim$1.8 & $\sim$-1.7    \\
  NJ                      & $\sim$1.6 & $\sim$-1.6    \\
  vL                      & $\sim$1.0 & $\sim$-6.3    \\
  \hline
  NL                      & $\sim$1.3 &  --           \\
  H  (if $L>4.5L_\odot$)   & $\sim$1.5 &  --           \\  
  H  (if $L\leq4.5L_\odot$)& $\sim$6.8 &  --           \\  
\end{tabular}


\end{center}
\end{table}

